MixDiT: Accelerating Image Diffusion Transformer Inference with Mixed-Precision MX Quantization

Diffusion Transformer (DiT) has driven significant progress in image generation tasks. However, DiT inferencing is notoriously compute-intensive and incurs long latency even on datacenter-scale GPUs, primarily due to its iterative nature and heavy reliance on GEMM operations inherent to its encoder-based structure. To address the challenge, prior work has explored quantization, but achieving low-precision quantization for DiT inferencing with both high accuracy and substantial speedup remains an open problem. To this end, this paper proposes MixDiT, an algorithm-hardware co-designed acceleration solution that exploits mixed Microscaling (MX) formats to quantize DiT activation values. MixDiT quantizes the DiT activation tensors by selectively applying higher precision to magnitude-based outliers, which produce mixed-precision GEMM operations. To achieve tangible speedup from the mixed-precision arithmetic, we design a MixDiT accelerator that enables precision-flexible multiplications and efficient MX precision conversions. Our experimental results show that MixDiT delivers a speedup of 2.10-5.32 times over RTX 3090, with no loss in FID.

==> body/acknowledgments.tex <==
\section*{Acknowledgments}
This should be a simple paragraph before the References to thank those individuals and institutions who have supported your work on this article.


==> body/relatedwork.tex <==
\vspace{-0.2cm}
\section{Related Work}

\textcolor{red}{
%
There have been algorithmic works aimed at applying quantization to image generation diffusion models, focusing on ``integer''  quantization with W8A8 or W4A8 bitwidths~\cite{qdit, viditq, ptq4dit}.
%
However, the lack of support for INT4$\times$INT8 kernels on GPUs and the high activation bitwidth limit the speedup. 
%
\sysname proposes a mixed-precision MX quantization scheme and its customized accelerator, offering substantially higher speedup.
}
% Image generation diffusion 모델을 PTQ 하겠다는 algorithm work 들이 있다. 
% diffusion transformer 양자화를 한 algorithm work 들 Q-DiT, ViDiT-Q, PTQ4DiT 는, W8A8 또는 W4A8 의 양자화를 하였다. 
% 하지만 GPU 에서 W4A8 kernel 의 부재와 높은 activation bitwidth로 인해, limited latency speedup 을 보였다. 
% 우리의 웍은 더 낮은 activation bitwidth 및 mixed-MX 연산 가속기를 제안함으로써 더 speedup 을 할 수 있음을 보였다. 
